A study of quasi-elastic muon neutrino and antineutrino scattering in the NOMAD experiment

We have studied the muon neutrino and antineutrino quasi-elastic (QEL) scattering reactions ($\nu_\mu n\to \mu^- p$ and $\bar{\nu}_\mu p\to \mu^+ n$) using a set of experimental data collected by the NOMAD collaboration. We have performed measurements of the cross-section of these processes on a nuclear target (mainly Carbon) normalizing it to the total $\nu_\mu$ ($\bar{\nu}_\mu$) charged current cross-section. The results for the flux averaged QEL cross-sections in the (anti)neutrino energy interval 3-100 GeV are $\sigma^{qel}_{\nu_\mu} = (0.92 \pm 0.02 (stat) \pm 0.06 (syst))\times 10^{-38} \cm^2$ and $\sigma{qel}_{\bar{\nu}_\mu} = (0.81 \pm 0.05 (stat) \pm 0.08 (syst))\times 10^{-38} \cm^2$ for neutrino and antineutrino, respectively. The axial mass parameter $M_A$ was extracted from the measured quasi-elastic neutrino cross-section. The corresponding result is $M_A = 1.05 \pm 0.02 (stat) \pm 0.06 (syst) GeV$. It is consistent with the axial mass values recalculated from the antineutrino cross-section and extracted from the pure $Q^2$ shape analysis of the high purity sample of $\nu_\mu$ quasi-elastic 2-track events, but has smaller systematic error and should be quoted as the main result of this work. Our measured $M_A$ is found to be in good agreement with the world average value obtained in previous deuterium filled bubble chamber experiments. The NOMAD measurement of $M_A$ is lower than those recently published by K2K and MiniBooNE collaborations. However, within the large errors quoted by these experiments on $M_A$, these results are compatible with the more precise NOMAD value.

==> tables/exp_anumu.tex <==
\begin{table*}[htb]
%\renewcommand{\arraystretch}{1.2}
\caption{\label{tab:ma_anumu}
The same as in Table~\ref{tab:ma_numu}, but for antineutrino experiments. The axial mass value for the NuTeV experiment~\cite{Suwonjandee:04} was estimated from the published antineutrino quasi-elastic cross section ($\sigma^{qel}_{\bar{\nu}}=(1.12\pm0.04(stat)\pm0.10(syst))\times 10^{-38}\,\cm^2$); systematic error for IHEP SKAT 90~\cite{Brunner:1989kw} is $0.20\,\GeV$. \hfill
}
\begin{tabular}{>{\em}l >{\em}l r >{$}r<{$}@{\hspace{5pt}}>{$}r<{$} >{\hspace{0pt}}c}
\hline\noalign{\smallskip}
\multicolumn{1}{l}{Experiment} & \multicolumn{1}{l}{Target} &
Events & \multicolumn{1}{r}{Determined from} & \multicolumn{1}{r}{$M_A,\,\GeV$} & {Ref.} \\
\noalign{\smallskip}\hline\noalign{\smallskip}
BNL 80       & Hydrogen  &        & \tdcs & \tnA{0.9^{+0.4}_{-0.3}}
                                  & \cite{Fanourakis:1980si} \\
BNL 88       & Liquid scint. & 2919 & \tdcs & \tnA{1.09 \pm 0.04}
                                  & \cite{Ahrens:1988rr} \\
\noalign{\smallskip}\hline\noalign{\smallskip}
FermiLab 84  & Neon      &    405 & \tdcs & \tnA{0.99\pm0.11}
                                  & \cite{Asratian:1984ir} \\
NuTeV 04     & Steel     &  15054 & \tcs  & \tnA{1.29 \pm 0.11}
                                  & \cite{Suwonjandee:04} \\
\noalign{\smallskip}\hline\noalign{\smallskip}
CERN GGM 77  & Freon     &    476 & \tlB & \tnB{0.69 \pm 0.44}{0.94 \pm 0.17}
                                  & \cite{Bonetti:1977cs} \\
CERN GGM 79 & Propane/Freon & 766 & \tlB & \tnB{0.84^{+0.08}_{-0.09}}{0.91 \pm 0.04}
                                  & \cite{Armenise:1979zg} \\
\noalign{\smallskip}\hline\noalign{\smallskip}
IHEP 85      & Aluminium    & 854 & d\sigma_{\nu+\bar{\nu}}/dQ^2 & \tnA{1.00 \pm 0.04}
                                  & \cite{Belikov:1983kg} \\
IHEP SKAT 88 & Freon        &  52 & \tlD & \tnA{0.72 \pm 0.23}
                                  & \cite{Grabosch:1986js} \\
IHEP SKAT 90 & Freon        &     & \tlC & \tnC{0.62\pm0.16}{0.79\pm0.11}{0.71\pm0.10}
                                  & \cite{Brunner:1989kw} \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table*}

